Semi-Supervised Learning from Small Annotated Data and Large Unlabeled Data for Fine-grained PICO Entity Recognition

Objective: Extracting PICO elements -- Participants, Intervention, Comparison, and Outcomes -- from clinical trial literature is essential for clinical evidence retrieval, appraisal, and synthesis. Existing approaches do not distinguish the attributes of PICO entities. This study aims to develop a named entity recognition (NER) model to extract PICO entities with fine granularities. Materials and Methods: Using a corpus of 2,511 abstracts with PICO mentions from 4 public datasets, we developed a semi-supervised method to facilitate the training of a NER model, FinePICO, by combining limited annotated data of PICO entities and abundant unlabeled data. For evaluation, we divided the entire dataset into two subsets: a smaller group with annotations and a larger group without annotations. We then established the theoretical lower and upper performance bounds based on the performance of supervised learning models trained solely on the small, annotated subset and on the entire set with complete annotations, respectively. Finally, we evaluated FinePICO on both the smaller annotated subset and the larger, initially unannotated subset. We measured the performance of FinePICO using precision, recall, and F1. Results: Our method achieved precision/recall/F1 of 0.567/0.636/0.60, respectively, using a small set of annotated samples, outperforming the baseline model (F1: 0.437) by more than 16\%. The model demonstrates generalizability to a different PICO framework and to another corpus, which consistently outperforms the benchmark in diverse experimental settings (p-value \textless0.001). Conclusion: This study contributes a generalizable and effective semi-supervised approach to named entity recognition leveraging large unlabeled data together with small, annotated data. It also initially supports fine-grained PICO extraction.

==> tables/suptable6_bak.tex <==

\begin{tabular}{*{8}{c}}
\toprule
\multicolumn{3}{c}{Basline Avg} & \multicolumn{3}{c}{Semi Avg}\\
\cmidrule(rl){1-3}\cmidrule(rl){4-6}
\textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{Model Type} & \textbf{Ontology} \\
\midrule
0.49 & 0.39 & 0.44 & 0.61 & 0.57 & 0.59 & In\_Domain & raw \\
0.67 & 0.60 & 0.63 & 0.67 & 0.62 & 0.65 & In\_Domain & raw \\
0.69 & 0.63 & 0.66 & 0.69 & 0.65 & 0.67 & In\_Domain & raw \\
0.69 & 0.63 & 0.66 & 0.70 & 0.66 & 0.68 & In\_Domain & raw \\
0.71 & 0.65 & 0.68 & 0.72 & 0.66 & 0.69 & In\_Domain & raw \\
0.49 & 0.39 & 0.44 & 0.62 & 0.58 & 0.60 & Cross\_Domain\_EBM & raw \\
0.67 & 0.60 & 0.63 & 0.67 & 0.62 & 0.64 & Cross\_Domain\_EBM & raw \\
0.69 & 0.63 & 0.66 & 0.70 & 0.65 & 0.67 & Cross\_Domain\_EBM & raw \\
0.69 & 0.63 & 0.66 & 0.70 & 0.65 & 0.67 & Cross\_Domain\_EBM & raw \\
0.71 & 0.65 & 0.68 & 0.73 & 0.67 & 0.70 & Cross\_Domain\_EBM & raw \\
0.72 & 0.66 & 0.69 & 0.72 & 0.68 & 0.70 & Cross\_Domain\_EBM & raw \\
\bottomrule
\end{tabular}%

\vspace{0.5cm}

\begin{tabular}{cccccccc}
\toprule
\textbf{Percent Anno} & \textbf{Recall pValue} & \textbf{Precision pValue} & \textbf{F1 pValue} & \textbf{Baseline Recall Avg} & \textbf{Semi Recall Avg} & \textbf{Model Type} & \textbf{Ontology} \\
\midrule
10 & 9.52E-32 & 2.82E-35 & 2.82E-34 & 0.49 & 0.61 & In\_Domain & raw \\
30 & 0.32 & 6.26E-15 & 5.84E-09 & 0.67 & 0.67 & In\_Domain & raw \\
50 & 0.97 & 1.02E-10 & 8.73E-06 & 0.69 & 0.69 & In\_Domain & raw \\
70 & 1.88E-07 & 1.15E-19 & 4.93E-16 & 0.69 & 0.70 & In\_Domain & raw \\
90 & 1E-3 & 2.96E-08 & 5.58E-07 & 0.71 & 0.72 & In\_Domain & raw \\
10 & 1.04E-36 & 1.85E-40 & 2.01E-39 & 0.49 & 0.62 & Cross\_Domain\_EBM & raw \\
30 & 0.05 & 3.57E-12 & 1.75E-08 & 0.67 & 0.67 & Cross\_Domain\_EBM & raw \\
50 & 1.50E-08 & 1.05E-12 & 7.79E-12 & 0.69 & 0.70 & Cross\_Domain\_EBM & raw \\
70 & 9.77E-10 & 9.42E-13 & 1.79E-12 & 0.69 & 0.70 & Cross\_Domain\_EBM & raw \\
90 & 2.54E-12 & 2.11E-12 & 4.98E-13 & 0.71 & 0.73 & Cross\_Domain\_EBM & raw \\
100 & 0.64 & 2.01E-08 & 1.48E-05 & 0.72 & 0.72 & Cross\_Domain\_EBM & raw \\
\bottomrule
\end{tabular}%
